Aeronautical Ad Hoc Networking for the Internet-Above-The-Clouds

The engineering vision of relying on the ``smart sky" for supporting air traffic and the ``Internet above the clouds" for in-flight entertainment has become imperative for the future aircraft industry. Aeronautical ad hoc Networking (AANET) constitutes a compelling concept for providing broadband communications above clouds by extending the coverage of Air-to-Ground (A2G) networks to oceanic and remote airspace via autonomous and self-configured wireless networking amongst commercial passenger airplanes. The AANET concept may be viewed as a new member of the family of Mobile ad hoc Networks (MANETs) in action above the clouds. However, AANETs have more dynamic topologies, larger and more variable geographical network size, stricter security requirements and more hostile transmission conditions. These specific characteristics lead to more grave challenges in aircraft mobility modeling, aeronautical channel modeling and interference mitigation as well as in network scheduling and routing. This paper provides an overview of AANET solutions by characterizing the associated scenarios, requirements and challenges. Explicitly, the research addressing the key techniques of AANETs, such as their mobility models, network scheduling and routing, security and interference are reviewed. Furthermore, we also identify the remaining challenges associated with developing AANETs and present their prospective solutions as well as open issues. The design framework of AANETs and the key technical issues are investigated along with some recent research results. Furthermore, a range of performance metrics optimized in designing AANETs and a number of representative multi-objective optimization algorithms are outlined.

==> LaTeXbib.tex <==
@article{alpcan2011security,
  title={{Security games for vehicular networks}},
  author={Alpcan, Tansu and Buchegger, Sonja},
  journal={IEEE Transactions on Mobile Computing},
  volume={10},
  number={2},
  pages={280--290},
  month={Ferbuary}, 
  year={2011},
  publisher={IEEE}
}
@article{ait2014spatio,
author={Ait Ali, K. and Baala, O. and Caminada, A}, 
journal={IEEE Transactions on Vehicular Technology}, 
title={{On the spatiotemporal traffic variation in vehicle mobility modeling}}, 
month={February}, 
year={2015}, 
volume={64}, 
number={2}, 
pages={652--667}, 
}
@article{akhtar2014vehicle,
  author={Akhtar, N. and Coleri Ergen, S. and Ozkasap, O.}, 
journal={IEEE Transactions on Vehicular Technology}, 
title={{Vehicle mobility and communication channel models for realistic and efficient highway VANET simulation}}, 
year={2015}, 
month={January}, 
volume={64}, 
number={1}, 
pages={248--262}, 
}
@article{al2012new,
  title={{A new scalable hybrid routing protocol for VANETs}},
  author={Al-Rabayah, Mohammad and Malaney, Robert},
  journal={IEEE Transactions on Vehicular Technology},
  volume={61},
  number={6},
  pages={2625--2635},	
  month={July}, 
  year={2012},
  publisher={IEEE}
}
@article{asefi2012mobility,
  title={{A mobility-aware and quality-driven retransmission limit adaptation scheme for video streaming over VANETs}},
  author={Asefi, Mahdi and Mark, Jon W and Shen, Xuemin},
  journal={IEEE Transactions on Wireless Communications},
  volume={11},
  number={5},
  pages={1817--1827},
  year={2012},
  publisher={IEEE}
}
@article{bai2010exploiting,
  title={{Exploiting the wisdom of the crowd: localized, distributed information-centric VANETs}},
  author={Bai, Fan and Krishnamachari, Bhaskar},
  journal={IEEE Communications Magazine},
  volume={48},
  number={5},
  pages={138--146},
  year={2010},
  publisher={IEEE}
}

@article{bharati2013cah,
  title={{CAH-MAC: cooperative ADHOC MAC for vehicular networks}},
  author={Bharati, Sailesh and Zhuang, Weihua},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={31},
  number={9},
  pages={470--479},
  year={2013},
  publisher={IEEE}
}

@article{blum2004threat,
  title={{The threat of intelligent collisions}},
  author={Blum, Jeremy and Eskandarian, Azim},
  journal={IT professional},
  volume={6},
  number={1},
  pages={24--29},
  year={2004},
  publisher={IEEE}
}

@article{bur2010wireless,
  title={{Wireless sensor and actuator networks: enabling the nervous system of the active aircraft}},
  author={Bur, Kaan and Omiyi, Peter and Yang, Yang},
  journal={IEEE Communications Magazine},
  volume={48},
  number={7},
  pages={118--125},
  year={2010},
  publisher={IEEE}
}

@article{chaintreau2007impact,
  title={{Impact of human mobility on opportunistic forwarding algorithms}},
  author={Chaintreau, Augustin and Hui, Pan and Crowcroft, Jon and Diot, Christophe and Gass, Richard and Scott, James},
  journal={IEEE Transactions on Mobile Computing},
  volume={6},
  number={6},
  pages={606--620},
  year={2007},
  publisher={IEEE}
}

@article{dietzel2013graph,
  title={{Graph-based metrics for insider attack detection in VANET multihop data dissemination protocols}},
  author={Dietzel, Stefan and Petit, Jonathan and Heijenk, Geert and Kargl, Frank},
  journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={4},
  pages={1505--1518},
  year={2013},
  publisher={IEEE}
}

@article{degardin2013theoretical,
  title={{Theoretical approach to the feasibility of power-line communication in aircrafts}},
  author={Degardin, Virginie and Junqua, I and Lienard, Martine and Degauque, Pierre and Bertuol, S},
  journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={3},
  pages={1362--1366},
  year={2013},
  publisher={IEEE}
}

@article{dhananjay2009practical,
  title={{Practical, distributed channel assignment and routing in dual-radio mesh networks}},
  author={Dhananjay, Aditya and Zhang, Hui and Li, Jinyang and Subramanian, Lakshminarayanan},
  journal={ACM SIGCOMM Computer Communication Review},
  volume={39},
  number={4},
  pages={99--110},
  year={2009},
  organization={ACM}
}

@article{dietzel2010resilient,
  title={{Resilient secure aggregation for vehicular networks}},
  author={Dietzel, Stefan and Schoch, Elmar and Konings, Bastian and Weber, Michael and Kargl, Frank},
  journal={IEEE Network},
  volume={24},
  number={1},
  pages={26--31},
  year={2010},
  publisher={IEEE}
}

@article{djukic2009delay,
  title={{Delay aware link scheduling for multi-hop TDMA wireless networks}},
  author={Djukic, Petar and Valaee, Shahrokh},
  journal={IEEE/ACM Transactions on Networking (TON)},
  volume={17},
  number={3},
  pages={870--883},
  year={2009},
  publisher={IEEE Press}
}

@article{ducourthial2007conditional,
  title={{Conditional transmissions: Performance study of a new communication strategy in VANET}},
  author={Ducourthial, Bertrand and Khaled, Yacine and Shawky, Mohamed},
  journal={IEEE Transactions on Vehicular Technology},
  volume={56},
  number={6},
  pages={3348--3357},
  year={2007},
  publisher={IEEE}
}

@article{eiza2013evolving,
  title={{An evolving graph-based reliable routing scheme for VANETs}},
  author={Eiza, Mahmoud Hashem and Ni, Qiang},
  journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={4},
  pages={1493--1504},
  year={2013},
  publisher={IEEE}
}

@article{ercetin2005modeling,
  title={{Modeling study for evaluation of aeronautical broadband data requirements over satellite networks}},
  author={Ercetin, Ozgur and Ball, Michael O and Tassiulas, Leandros},
  journal={IEEE Transactions on Aerospace and Electronic Systems},
  volume={41},
  number={1},
  pages={361--370},
  year={2005},
  publisher={IEEE}
}

@article{fiore2013persistent,
  title={{Persistent localized broadcasting in VANETs}},
  author={Fiore, Marco and Casetti, Claudio and Chiasserini, Carla-Fabiana and Borsetti, Diego},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={31},
  number={9},
  pages={480--490},
  year={2013},
  publisher={IEEE}
}

@article{gfeller1979wireless,
  title={{Wireless in-house data communication via diffuse infrared radiation}},
  author={Gfeller, Fritz R and Bapst, Urs},
  journal={Proceedings of the IEEE},
  volume={67},
  number={11},
  pages={1474--1486},
  year={1979},
  publisher={IEEE}
}

@article{giordano2011corner,
  title={{Corner: a radio propagation model for VANETs in urban scenarios}},
  author={Giordano, Eugenio and Frank, Raphael and Pau, Giovanni and Gerla, Mario},
  journal={Proceedings of the IEEE},
  volume={99},
  number={7},
  pages={1280--1294},
  year={2011},
  publisher={IEEE}
}

@article{hao2013secure,
  title={{Secure cooperative data downloading in vehicular ad hoc networks}},
  author={Hao, Yong and Tang, Jin and Cheng, Yu},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={31},
  number={9},
  pages={523--537},
  year={2013},
  publisher={IEEE}
}

@article{harri2009mobility,
  title={{Mobility models for vehicular ad hoc networks: a survey and taxonomy}},
  author={Harri, Jerome and Filali, Fethi and Bonnet, Christian},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={11},
  number={4},
  pages={19--41},
  year={2009},
  publisher={IEEE}
}

@article{hsu2005weighted,
  title={{Weighted waypoint mobility model and its impact on ad hoc networks}},
  author={Hsu, Wei-jen and Merchant, Kashyap and Shu, Haw-wei and Hsu, Chih-hsin and Helmy, Ahmed},
  journal={ACM SIGMOBILE Mobile Computing and Communications Review},
  volume={9},
  number={1},
  pages={59--63},
  year={2005},
  publisher={ACM}
}

@article{huang2009performance,
  title={{Performance study of node-disjoint multipath routing in vehicular ad hoc networks}},
  author={Huang, Xiaoxia and Fang, Yuguang},
  journal={IEEE Transactions on Vehicular Technology},
  volume={58},
  number={4},
  pages={1942--1950},
  year={2009},
  publisher={IEEE}
}

@article{hunukumbure2007radio,
  title={{Radio network dimensioning and planning for WiMAX networks}},
  author={Hunukumbure, VBUVM and Vadgama, V},
  journal={Fujitsu Scientific \& Technical Journal},
  volume={43},
  number={4},
  pages={435--450},
  year={2007}
}

@article{hwang2008intent,
  title={{Intent-based probabilistic conflict detection for the next generation air transportation system}},
  author={Hwang, Inseok and Seah, Chze Eng},
  journal={Proceedings of the IEEE},
  volume={96},
  number={12},
  pages={2040--2059},
  year={2008},
  publisher={IEEE}
}

@article{isaac2010security,
  title={{Security attacks and solutions for vehicular ad hoc networks}},
  author={Isaac, Jes{\'u}s T{\'e}llez and Zeadally, Sherali and C{\'a}mara, Jos{\'e} Sierra},
  journal={IET Communications},
  volume={4},
  number={7},
  pages={894--903},
  year={2010},
  publisher={IET}
}

@article{jang2012location,
  title={{Location-based TDMA MAC for reliable aeronautical communications}},
  author={Jang, Hyungjun and Kim, Eunkyung and Lee, Jae-Joon and Lim, Jaesung},
  journal={IEEE Transactions on Aerospace and Electronic Systems},
  volume={48},
  number={2},
  pages={1848--1854},
  year={2012},
  publisher={IEEE}
}

@article{jeong2013intervehicle,
  title={{Intervehicle communication: cox-fox modeling}},
  author={Jeong, Youngmin and Jo Chong, W and Shin, Hyundong and Win, M},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={31},
  number={9},
  pages={418--433},
  year={2013},
  publisher={IEEE}
}

@article{jerbi2009towards,
  title={{Towards efficient geographic routing in urban vehicular networks}},
  author={Jerbi, Moez and Senouci, S-M and Rasheed, Tinku and Ghamri-Doudane, Yacine},
  journal={IEEE Transactions on Vehicular Technology},
  volume={58},
  number={9},
  pages={5048--5059},
  year={2009},
  publisher={IEEE}
}

@article{katti2008symbol,
  title={{Symbol-level network coding for wireless mesh networks}},
  author={Katti, Sachin and Katabi, Dina and Balakrishnan, Hari and Medard, Muriel},
  journal={ACM SIGCOMM Computer Communication Review},
  volume={38},
  number={4},
  pages={401--412},
  year={2008},
  organization={ACM}
}

@article{kerns1991data,
  title={{Data-link communication between controllers and pilots: a review and synthesis of the simulation literature}},
  author={Kerns, Karol},
  journal={The International Journal of Aviation Psychology},
  volume={1},
  number={3},
  pages={181--204},
  year={1991},
  publisher={Taylor \& Francis}
}


@article{khabazian2008performance,
  title={{A performance modeling of connectivity in vehicular ad hoc networks}},
  author={Khabazian, Mehdi and Ali, Mustafa K Mehmet},
  journal={IEEE Transactions on Vehicular Technology},
  volume={57},
  number={4},
  pages={2440--2450},
  year={2008},
  publisher={IEEE}
}

@article{khabazian2011performance,
  title={{Performance modeling of message dissemination in vehicular ad hoc networks with priority}},
  author={Khabazian, Mehdi and Aissa, Sonia and Mehmet-Ali, Mustafa},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={29},
  number={1},
  pages={61--71},
  year={2011},
  publisher={IEEE}
}

@article{knorr2012reducing,
  title={{Reducing traffic jams via VANETs}},
  author={Knorr, Florian and Baselt, Daniel and Schreckenberg, Michael and Mauve, Martin},
  journal={IEEE Transactions on Vehicular Technology},
  volume={61},
  number={8},
  pages={3490--3498},
  year={2012},
  publisher={IEEE}
}

@article{kosch2006scalability,
  title={{The scalability problem of vehicular ad hoc networks and how to solve it}},
  author={Kosch, Timothy and Adler, Christian J and Eichler, Stephan and Schroth, Christoph and Strassberger, Markus},
  journal={IEEE Wireless Communications},
  volume={13},
  number={5},
  pages={22--28},
  year={2006},
  publisher={IEEE}
}

@article{kounga2009proving,
  title={{Proving reliability of anonymous information in VANETs}},
  author={Kounga, Gina and Walter, Thomas and Lachmund, Sven},
  journal={IEEE Transactions on Vehicular Technology},
  volume={58},
  number={6},
  pages={2977--2989},
  year={2009},
  publisher={IEEE}
}

@article{lee2010survey,
  title={{Survey of routing protocols in vehicular ad hoc networks}},
  author={Lee, Kevin C and Lee, Uichin and Gerla, Mario},
  journal={Advances in vehicular ad-hoc networks: Developments and challenges},
  pages={149--170},
  year={2010},
  publisher={Information Science Reference (IGI Global)}
}

@article{lee2010fleanet,
  title={{FleaNet: a virtual market place on vehicular networks}},
  author={Lee, Uichin and Lee, Jiyeon and Park, Joon-Sang and Gerla, Mario},
  journal={IEEE Transactions on Vehicular Technology},
  volume={59},
  number={1},
  pages={344--355},
  year={2010},
  publisher={IEEE}
}

@article{leinmuller2006position,
  title={{Position verification approaches for vehicular ad hoc networks}},
  author={Leinmuller, Tim and Schoch, Elmar and Kargl, Frank},
  journal={IEEE Wireless Communications},
  volume={13},
  number={5},
  pages={16--21},
  year={2006},
  publisher={IEEE}
}

@article{li2013inter,
  title={{Inter-node mobility correlation for group detection and analysis in VANETs}},
  author={Li, Yujin and Zhao, Ming and Wang, Wenye}, 
journal={IEEE Transactions on Vehicular Technology}, 
year={2013}, 
volume={62}, 
number={9}, 
pages={4590-4601}, 
}

@article{lin2013achieving,
  title={{Achieving efficient cooperative message authentication in vehicular ad hoc networks}},
  author={Lin, Xiaodong and Li, Xu},
  journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={7},
  pages={3339--3348},
  year={2013},
  publisher={IEEE}
}

@article{liu2009vgsim,
  title={{VGSim: an integrated networking and microscopic vehicular mobility simulation platform}},
  author={Liu, Bojin and Khorashadi, Behrooz and Du, Haining and Ghosal, Dipak and Chuah, Chen-Nee and Zhang, Michael},
  journal={IEEE Communications Magazine},
  volume={47},
  number={5},
  pages={134--141},
  year={2009},
  publisher={IEEE}
}

@article{lu2013lightweight,
  title={{A lightweight conditional privacy-preservation protocol for vehicular traffic-monitoring systems}},
  author={Lu, Rongxing and Lin, Xiaodong and Shi, Zhiguo and Xuemin (Sherman) Shen},
  journal={IEEE Intelligent Systems},
  volume={28},
  number={3},
  pages={62--65},
  year={2013}
}

@article{ma2012design,
  title={{Design and analysis of a robust broadcast scheme for VANET safety-related services}},
  author={Ma, Xiaomin and Zhang, Jinsong and Yin, Xiaoyan and Trivedi, Kishor S},
  journal={IEEE Transactions on Vehicular Technology},
  volume={61},
  number={1},
  pages={46--61},
  year={2012},
  publisher={IEEE}
}

@article{maihofer2004survey,
  title={{A survey of geocast routing protocols}},
  author={Maihofer, Christian},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={6},
  number={2},
  pages={32--42},
  year={2004},
  publisher={IEEE}
}

@article{mayer2009trends,
  title={Trends in aeronautical flight test telemetry},
  author={Mayer, Gerhard and Chalfant, Timothy},
  journal={Journal of Aerospace Science and Technologies},
  volume={61},
  number={1},
  pages={252},
  year={2009}
}
@article{mohimani2009mobility,
  title={{Mobility modeling, spatial traffic distribution, and probability of connectivity for sparse and dense vehicular ad hoc networks}},
  author={Mohimani, G Hosein and Ashtiani, Farid and Javanmard, Adel and Hamdi, Maziyar},
  journal={IEEE Transactions on Vehicular Technology},
  volume={58},
  number={4},
  pages={1998--2007},
  year={2009},
  publisher={IEEE}
}

@article{narlikar2010designing,
  title={{Designing multihop wireless backhaul networks with delay guarantees}},
  author={Narlikar, Girija and Wilfong, Gordon and Zhang, Lisa},
  journal={Wireless Networks},
  volume={16},
  number={1},
  pages={237--254},
  year={2010},
  publisher={Springer-Verlag New York, Inc.}
}

@article{nelson1985spatial,
  title={Spatial TDMA: a collision-free multihop channel access protocol},
  author={Nelson, Randolph and Kleinrock, Leonard},
  journal={Communications, IEEE Transactions on},
  volume={33},
  number={9},
  pages={934--944},
  year={1985},
  publisher={IEEE}
}

@article{omar2013vemac,
  title={{VeMAC: a TDMA-based MAC protocol for reliable broadcast in VANETs}},
  author={Omar, Hassan Aboubakr and Zhuang, Weihua and Li, Li},
  journal={IEEE Transactions on Mobile Computing},
  volume={12},
  number={9},
  pages={1724--1736},
  year={2013},
  publisher={IEEE}
}

@article{panichpapiboon2012review,
  title={{A review of information dissemination protocols for vehicular ad hoc networks}},
  author={Panichpapiboon, Sooksan and Pattara-Atikom, Wasan},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={14},
  number={3},
  pages={784--798},
  year={2012},
  publisher={IEEE}
}

@article{papadimitratos2008secure,
  title={{Secure vehicular communication systems: design and architecture}},
  author={Papadimitratos, Panagiotis and Buttyan, Levente and Holczer, Tam{\'a}s and Schoch, Elmar and Freudiger, Julien and Raya, Maxim and Ma, Zhendong and Kargl, Frank and Kung, Antonio and Hubaux, J-P},
  journal={IEEE Communications Magazine},
  volume={46},
  number={11},
  pages={100--109},
  year={2008},
  publisher={IEEE}
}

@article{patankar2004model,
  title={{A model for fault-tolerant networked control system using TTP/C communication}},
  author={Patankar, Ravindra P},
  journal={IEEE Transactions on Vehicular Technology},
  volume={53},
  number={5},
  pages={1461--1467},
  year={2004},
  publisher={IEEE}
}

@article{pogkas2007architecture,
  title={{Architecture design and implementation of an ad-hoc network for disaster relief operations}},
  author={Pogkas, Nikos and Karastergios, George E and Antonopoulos, Christos P and Koubias, Stavros and Papadopoulos, George},
  journal={IEEE Transactions on Industrial Informatics},
  volume={3},
  number={1},
  pages={63--72},
  year={2007},
  publisher={IEEE}
}

@article{qiu2011enhancing,
  title={{Enhancing the performance of video streaming in wireless mesh networks}},
  author={Qiu, Xiaoling and Liu, Haiping and Ghosal, Dipak and Mukherjee, Biswanath and Benko, John and Li, Wei and Bajaj, Rashmi},
  journal={Wireless Personal Communications},
  volume={56},
  number={3},
  pages={535--557},
  year={2011},
  publisher={Springer}
}

@article{rak2014lla,
  title={{LLA: a new anypath routing scheme providing long path lifetime in VANETs}},
  author={Rak, Jacek},
journal={IEEE Communications Letters},
  volume={18},
  number={2},
  pages={281--284},
  year={2014}
}


@article{saleet2010region,
  title={{Region-based location-service-management protocol for VANETs}},
  author={Saleet, Hanan and Basir, Otman and Langar, Rami and Boutaba, Raouf},
  journal={IEEE Transactions on Vehicular Technology},
  volume={59},
  number={2},
  pages={917--931},
  year={2010},
  publisher={IEEE}
}

@article{santi2005critical,
  title={{The critical transmitting range for connectivity in mobile ad hoc networks}},
  author={Santi, Paolo},
  journal={IEEE Transactions on Mobile Computing},
  volume={4},
  number={3},
  pages={310--317},
  year={2005},
  publisher={IEEE}
}

@article{schnell2007newsky,
  title={{Newsky-concept for networking the sky for civil aeronautical communications}},
  author={Schnell, Michael and Scalise, S},
  journal={IEEE Aerospace and Electronic Systems Magazine},
  volume={22},
  number={5},
  pages={25--29},
  year={2007},
  publisher={IEEE}
}

@article{segata2013automatic,
  title={{Automatic emergency braking: realistic analysis of car dynamics and network performance}},
  author={Segata, Michele and Lo Cigno, Renato},
 journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={9},
  pages={4150--4161},
  year={2013},
  publisher={IEEE}
}

@article{sofra2011route,
  title={{Route construction for long lifetime in VANETs}},
  author={Sofra, Nikoletta and Gkelias, Athanasios and Leung, Kin K},
  journal={IEEE Transactions on Vehicular Technology},
  volume={60},
  number={7},
  pages={3450--3461},
  year={2011},
  publisher={IEEE}
}

@article{sommer2008progressing,
  title={{Progressing toward realistic mobility models in VANET simulations}},
  author={Sommer, Christoph and Dressler, Falko},
  journal={IEEE Communications Magazine},
  volume={46},
  number={11},
  pages={132--137},
  year={2008},
  publisher={IEEE}
}

@article{soto2009nemo,
  title={{NEMO-enabled localized mobility support for internet access in automotive scenarios}},
  author={Soto, Ignacio and Bernardos, Carlos J and Calderon, Maria and Banchs, Albert and Azcorra, Arturo},
  journal={IEEE Communications Magazine},
  volume={47},
  number={5},
  pages={152--159},
  year={2009},
  publisher={IEEE}
}


@article{sun2011rescueme,
  title={{RescueMe: location-based secure and dependable VANETs for disaster rescue}},
  author={Sun, Jinyuan and Zhu, Xiaoyan and Zhang, Chi and Fang, Yuguang},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={29},
  number={3},
  pages={659--669},
  year={2011},
  publisher={IEEE}
}


@article{taleb2007stable,
  title={{A stable routing protocol to support ITS services in VANET networks}},
  author={Taleb, Tarik and Sakhaee, Ehssan and Jamalipour, Abbas and Hashimoto, Kazuo and Kato, Nei and Nemoto, Yoshiaki},
  journal={IEEE Transactions on Vehicular Technology},
  volume={56},
  number={6},
  pages={3337--3347},
  year={2007},
  publisher={IEEE}
}

@article{toor2008vehicle,
  title={{Vehicle ad hoc networks: applications and related technical issues}},
  author={Toor, Yasser and Muhlethaler, Paul and Laouiti, Anis},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={10},
  number={3},
  pages={74--88},
  year={2008},
  publisher={IEEE}
}

@article{toutouh2012intelligent,
  title={{Intelligent OLSR routing protocol optimization for VANETs}},
  author={Toutouh, Jamal and Garc{\'\i}a-Nieto, Jos{\'e} and Alba, Enrique},
  journal={IEEE Transactions on Vehicular Technology},
  volume={61},
  number={4},
  pages={1884--1894},
  year={2012},
  publisher={IEEE}
}

@article{tsertou2008revisiting,
  title={{Revisiting the hidden terminal problem in a CSMA/CA wireless network}},
  author={Tsertou, Athanasia and Laurenson, David I},
  journal={IEEE Transactions on Mobile Computing},
  volume={7},
  number={7},
  pages={817--831},
  year={2008},
  publisher={IEEE}
}

@article{Venkatesh2014Routing,
  title={{Routing protocols for vehicular ad hoc networks (VANETs): a Review}},
  author={Venkatesh and Indra, A and Murali, R},
  journal={Journal of Emerging Trends in Computing and Information Sciences},
  volume={5},
  number={1},
  pages={25--43},
  year={2014}
}

@article{viriyasitavat2011uv,
  title={{UV-CAST: an urban vehicular broadcast protocol}},
  author={Viriyasitavat, W and Tonguz, OK and Bai, Fan},
  journal={IEEE Communications Magazine},
  volume={49},
  number={11},
  pages={116--124},
  year={2011},
  publisher={IEEE}
}

@article{wang2009small,
  title={{Small-scale and large-scale routing in vehicular ad hoc networks}},
  author={Wang, Wenjing and Xie, Fei and Chatterjee, Mainak},
  journal={IEEE Transactions on Vehicular Technology},
  volume={58},
  number={9},
  pages={5200--5213},
  year={2009},
  publisher={IEEE}
}

@article{wisitpongphan2007routing,
  title={{Routing in sparse vehicular ad hoc wireless networks}},
  author={Wisitpongphan, Nawaporn and Bai, Fan and Mudalige, Priyantha and Sadekar, Varsha and Tonguz, Ozan},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={25},
  number={8},
  pages={1538--1556},
  year={2007},
  publisher={IEEE}
}
	
@article{wong2008optical,
  title={{Optical design and multipath analysis for broadband optical wireless in an aircraft passenger cabin application}},
  author={Wong, Damon Wing Kee and Chen, George},
  journal={IEEE Transactions on Vehicular Technology},
  volume={57},
  number={6},
  pages={3598--3606},
  year={2008},
  publisher={IEEE}
}

@article{wu2013flexible,
  title={{Flexible, portable and practicable solution for routing in VANETs: a fuzzy constraint Q-learning approach}},
  author={Wu, Celimuge and Ohzahata, Satoshi and Kato, Toshihiko},
 journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={9},
  pages={4251--4263},
  year={2013},
  publisher={IEEE}
}

@article{zhang2012multicast,
  title={{Multicast capacity for VANETs with directional antenna and delay constraint}},
  author={Zhang, Guanglin and Xu, Youyun and Wang, Xinbing and Tian, Xiaohua and Liu, Jing and Gan, Xiao Yin and Yu, Hui and Qian, Liang},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={30},
  number={4},
  pages={818--833},
  year={2012},
  publisher={IEEE}
}


@article{zhu2011mobility,
  title={{Mobility and handoff management in vehicular networks: a survey}},
  author={Zhu, Kun and Niyato, Dusit and Wang, Ping and Hossain, Ekram and In Kim, Dong},
  journal={Wireless communications and mobile computing},
  volume={11},
  number={4},
  pages={459--476},
  year={2011},
  publisher={Wiley Online Library}
}
